Persistence of Conley-Morse Graphs in Combinatorial Dynamical Systems

Multivector fields provide an avenue for studying continuous dynamical systems in a combinatorial framework. There are currently two approaches in the literature which use persistent homology to capture changes in combinatorial dynamical systems. The first captures changes in the Conley index, while the second captures changes in the Morse decomposition. However, such approaches have limitations. The former approach only describes how the Conley index changes across a selected isolated invariant set though the dynamics can be much more complicated than the behavior of a single isolated invariant set. Likewise, considering a Morse decomposition omits much information about the individual Morse sets. In this paper, we propose a method to summarize changes in combinatorial dynamical systems by capturing changes in the so-called Conley-Morse graphs. A Conley-Morse graph contains information about both the structure of a selected Morse decomposition and about the Conley index at each Morse set in the decomposition. Hence, our method summarizes the changing structure of a sequence of dynamical systems at a finer granularity than previous approaches.

==> removed-Amorsedecomps.tex <==
\section{Morse Decompositions}

\subsection{Minimal Morse Decompositions}
\label{appendix:minimal-morse-decomps}


\begin{proposition}
Let $S$ denote an isolated invariant set in $N$, and let $\md{}$ denote the set of minimal isolated invariant sets $M \subseteq S$. The set $\md{}$ is a Morse decomposition of $S$. 
\end{proposition}
\begin{proof}
Consider $\sigma \in S \setminus \left( \bigcup_{M \in \md{}}( M ) \right)$. Because $S$ is an invariant set, there must exist some essential solution $\rho \; : \; \mathbb{Z} \to S$ where $\rho( 0 ) = \sigma$. Proposition \ref{prop:alpha-omega-strongly-connected} implies that $\alpha( \rho )$ and $\omega( \rho )$ are strongly connected. Hence, $\alpha( \rho ) \subseteq M_1 \in \md{}$ while $\omega( \rho ) \subseteq M_2 \in \md{}$. This induces a relation $\leq$ on $\md{}$, and in this case we have that $M_2 \leq M_1$. It remains to be shown that $\leq$ is a partial order. 

First, we show that $\leq$ is reflexive. Note that each $M \in \md{}$ is an isolated invariant set, so there exists an essential solution $\rho \; : \; \mathbb{Z} \to S$ where $\rho( \mathbb{Z} ) \subseteq S$. Hence, $\alpha( \rho ) = \omega( \rho ) = M$, which implies $M \leq M$. 

Now, we show that $\leq$ is antisymmetric. Assume there exist $M_1, M_2 \in \md{}$ such that $M_1 \leq M_2$ and $M_2 \leq M_1$. Then there exist essential solutions $\rho, \rho' \; : \; \mathbb{Z} \to S$ such that $\alpha( \rho ) = \omega( \rho' ) = M_1$ and $\alpha( \rho' ) = \omega( \rho ) = M_2$. This implies that there exists a path from $M_1$ to $M_2$ and a path from $M_2$ to $M_1$. Since $M_2$ is strongly connected, this implies that there is a path from $M_1$ to itself. Since $M_1$ is isolated, it follows that $M_2 \subseteq M_1$. But elements of $\md{}$ are disjoint, so $M_1 = M_2$.  

Now, we show that $\leq$ is transitive. Assume that $M_1 \leq M_2$ and $M_2 \leq M_3$. Then there exist essential solutions $\rho, \rho' \; : \; \mathbb{Z} \to S$ such that $\alpha(\rho) = M_2$, $\omega(\rho) = M_1$, $\alpha( \rho' ) = M_3$, and $\omega(\rho') = M_2$. By truncating and concatenating $\rho$ and $\rho'$, and taking advantage of the fact that $M_2$ is strongly connected, it is easy to construct an essential solution $\rho'' \; : \; \mathbb{Z} \to S$ such that $\alpha(\rho'' ) = M_3$ and $\omega( \rho'' ) = M_1$. Thus, $M_1 \leq M_3$.

Hence, $\md{}$ is a Morse decomposition for $S$, as $N$ and $\leq$ satisfy the requisite criteria. 
\end{proof}

\subsection{Minimal and Strongly Connected Isolated Invariant Sets}
\label{appendix:strongly-connected}

In this section, we give a proof for Proposition \ref{prop:min}. This result is very similar to a result in \cite{DJKKLM19}, but the result in \cite{DJKKLM19} uses a different definition of an invariant set. Hence, we reprove it for completeness. We begin with the notion of a strongly connected invariant set. 

\begin{definition}
Let $\mv{}$ denote a multivector, and let $S$ denote an invariant set in $N$. The isolated invariant set $S$ is \emph{strongly connected} if for all $\sigma,\tau \in S$, there exists a path $\rho \; : \; \mathbb{Z} \cap [0,n] \to S$ where $\rho(0) = \sigma$ and $\rho(n) = \tau$. 
\end{definition}

We first aim to show that a minimal isolated invariant set $S$ is strongly connected. 

\begin{proposition}
Let $S$ denote an isolated invariant set in $N$. If $S$ is strongly connected, then $S$ is minimal.  
\end{proposition}
\begin{proof}
We proceed by showing the contrapositive: if $S$ is not minimal, then $S$ is not strongly connected. If $S$ is not minimal, then there exists some Morse decomposition $\md{}$ for $S$. Hence, there exists a closed set $N$ that isolates $S$ and all $M \in \md{}$. In addition, there is a partial order $\leq$ on $\md{}$ where $M \leq M'$ if and only if there is a path from $M' \in \md{}$ to $M \in \md{}$. As $S$ is not minimal, $|\md{}| \geq 2$. Hence, consider $M_1, M_2 \in \md{}$, $M_1 \neq M_2$. Then we have three cases: $M_1$ and $M_2$ are not related by $\leq$, $M_1 \leq M_2$, or $M_2 \leq M_1$. If $M_1$ and $M_2$ are not related, then there does not exist a path from some $\sigma \in M_1$ to $\tau \in M_2$, or vice-versa. Hence, in this case, $S$ is clearly not strongly connected. In the case where $M_1 \leq M_2$, there exists a path from $\tau \in M_2$ to $\sigma \in M_1$. If there exists a path from $\sigma$ to $\tau$, then $M_2 \leq M_1$. By the antisymmetry of $\leq$, it follows that $M_1 = M_2$, a contradiction. Hence, there can exist no path from $\tau$ to $\sigma$. This implies that $S$ is not strongly connected. In the case where $M_2 \leq M_1$, we get that $S$ is not strongly connected by identical reasoning.
\end{proof}

The reverse direction is more difficult. To prove it, we require the notion of the isolated completion. 
\begin{definition}
Let $S$ be an invariant set in a closed set $N$. The \emph{isolated completion} of $S$ in $N$ is the smallest isolated invariant set $S'$ in $N$ such that $S \subseteq S'$.
\end{definition}
Note that the isolated completion of $S$ may be different depending on the chosen $N$.
\begin{proposition}
Let $S$ be an invariant set in $N$. Then $\iscomp_N(S) = S \cup R$, where $R$ is the is the union of the images of all paths $\rho \; : \; \mathbb{Z}\cap[0,n] \to N$ where $\rho(0), \rho(n) \in S$ and $\rho(i)\not\in S$ for all $i \in (0,n) \cap \mathbb{Z}$. 
\label{prop:iscomp-paths}
\end{proposition}
\begin{proof}
Note that $\iscomp_N(S)$ necessarily contains $S$, and if there exists a $\rho \; : \; \mathbb{Z}\cap[0,n] \to N$ such that $\rho(0), \rho(n) \in S$ and $\im( \rho ) \not\subset \iscomp_N(S)$, then $\iscomp_N(S)$ is not isolated. Axiomatically, each $\sigma \in S$ is part of an essential solution that is contained in $S$. If $\sigma = \rho(i)$, then we construct an essential solution $\rho'$ such that $\rho'(i) = \sigma$. As $\rho( 0 ),\rho(n) \in S$, there must exist essential solutions $r_0, r_n \; : \; \mathbb{Z} \to S$ such that $r_0( 0 ) = \rho(0)$ and $r_n( n ) = \rho(n)$. Thus, we let $\rho'(j) := r_0(j)$ if $j \leq 0$, $\rho'(j) = \rho( j )$ if $0 \leq j \leq n$, and $\rho'(n) = r_n(j)$ if $j \geq n$. Thus, $\sigma = \rho'(i)$, so $S \cup R$ is an invariant set. Thus, we have shown that $S \cup R$ is the smallest isolated invariant set which contains $S$, so $\iscomp_N(S) = S \cup R$. 
\end{proof}

We are in particular interested in the case of the minimal Morse decomposition.

\begin{proposition}
Let $S \subseteq N$ denote an invariant set, and let $S'$ denote an isolated invariant set in $N$. If $S \subseteq S'$, then $\iscomp_N(S) \subseteq S'$. 
\label{prop:is-comp-included}
\end{proposition}
\begin{proof}
By Proposition \ref{prop:iscomp-paths}, $\iscomp_N(S) = S \cup R$, where $R$ is the set of paths in $N$ which originate and terminate in $S$. Consider such a path $\rho \; : \; [0,n] \cap \mathbb{Z} \to N$, where $\rho(0) \in S \subseteq S'$ and $\rho( n ) \in S \subseteq S'$. By assumption, $S'$ is isolated, so it follows that for all $i \in [0,n] \cap \mathbb{Z}$, $\rho(i) \in S'$. Hence, $S \subseteq S'$ and $R \subseteq S'$, so it follows that $\iscomp_N( S ) \subseteq S'$. 
\end{proof}


\begin{proposition}
Let $S$ denote a strongly connected invariant set in $N$. The isolated invariant set $\iscomp_N(S)$ is strongly connected.
\label{prop:isolated-completion-strongly-connected}
\end{proposition}
\begin{proof}
By Proposition \ref{prop:iscomp-paths}, $\iscomp_N(S) = S \cup R$, where $R$ is the union of the images of paths $\rho \; : \; \mathbb{Z} \cap [0,n] \to N$ such that $\rho(0),\rho(n) \in S$. Hence, let $r$ denote a simplex on such a path $\rho$. By concatenating paths, there exists a path in $\iscomp_N(S)$ from all $\sigma \in S$ to $r$ and there exists a path in $\iscomp_N(S)$ from $r$ to all $\sigma \in S$. Hence, by again composing paths, there exists a path from all $r \in R$ to all $r' \in R$. Thus, it follows immediately that $\iscomp_N(S)$ is strongly connected. 
\end{proof}

\begin{proposition}
Let $\sigma$ denote a simplex, and let $\rho \; : \; \mathbb{Z} \to K$ denote an essential solution where $\rho( 0 ) = \sigma$. The sets $\alpha( \rho )$ and $\omega( \rho )$ are strongly connected invariant sets.
\label{prop:alpha-omega-strongly-connected}
\end{proposition}
\begin{proof}
We will show that $\alpha( \rho )$ is a strongly connected invariant set, and the result for $\omega( \rho )$ follows analogously. We claim that there must exist some path $\rho' \; : \; [a,b]\cap\mathbb{Z} \to K$ such that $\rho'(i) = \rho(i)$ for all $i \in [a,b] \cap \mathbb{Z}$, $\rho'(a) = \rho'(b)$, and $\im(\rho') = \alpha$. To show this, we first show that there must exist a $j < 0$ such that $\rho(-\infty,j] = \alpha(\rho)$. Clearly,  $\alpha( \rho ) \subseteq \rho(-\infty,j]$ for all $j$, because $\alpha( \rho ) = \bigcap_{i=1}^\infty \rho(-\infty,-i]$. Hence, note that for each $\sigma \in K \setminus \alpha(\rho)$, there must exist some maximum $j' < 0$ such that $\sigma \not\in \rho( -\infty, j]$. Take $j$ to be the minimum of all such $j'$, and it follows immediately that $\rho(-\infty, j] = \alpha(\rho)$. To construct $\rho'$, pick an arbitrary index $\sigma \in \alpha(\rho)$, and pick a $b < j$ such that $\rho( k ) = \sigma$. Note that such a $b$ must exist, else $\sigma \not\in \alpha(\rho)$. Similarly, for each $\tau \in \alpha( \rho ) \setminus \{ \sigma \}$, there must exist an index $b' < b$ such that $\rho( b' ) = \tau$. Again, there must exist an index $a$ less than all such $b'$ such that $\rho( a ) = \sigma$. This choice of $a$ and $b$ gives us $\rho' \; : \; [a,b] \cap \mathbb{Z} \to K$ such that $\im( \rho' ) = \alpha( \rho' )$ and $\rho'(a) = \rho'(b) = \sigma$. This gives a canonical path between any $\tau_1$ and $\tau_2$ in $\alpha( \rho )$: $\rho'$ gives a path from $\tau_1$ to $\sigma$ and a path from $\sigma$ to $\tau_2$, which gives a path from $\tau_1$ to $\tau_2$. 
\end{proof}

\begin{proposition}
Let $S$, denote an isolated invariant set in $N$. If there exists a strongly connected isolated invariant set $S' \subsetneq S$ in $N$, then there exists a Morse decomposition $\md{}$ for $S$ where $|\md{}| \geq 2$. 
\label{prop:morse-decomp-exists}
\end{proposition}
\begin{proof}
We begin by considering three sets of simplices, denoted $F(S')$, $B(S')$, and $U(S')$. The set $F(S')$ is taken to be the set of simplices $\sigma$ in $S \setminus S'$ for which there exists a path in $S$ from some $\tau \in S'$ to $\sigma$, and $B(S)$ is taken to be the set of simplices $\sigma$ in $S \setminus S'$ for which there exists a path in $S$ from $\sigma$ to some $\tau \in S'$. We take $N(S)$ to be $S \setminus ( B(S') \cup F(S') \cup S')$. Equivalently, $N(S')$ is the set of simplices $\sigma$ in $S \setminus S'$ for which there does not exist a $\tau \in S'$ such that there is a path from $\sigma$ to $\tau$ or from $\tau$ to $\sigma$. It is easy to see that $B(S') \cap F(S') = \emptyset$. If there was a $\sigma \in B(S') \cap F(S')$, then there necessarily exists a path from $S'$ to $\sigma$ and from $\sigma$ to $S'$, which implies that $S$ is not isolated, a contradiction.  By construction, $N(S') \cap F(S') = \emptyset$ and $N(S') \cap B(S') = \emptyset$, so all three sets are disjoint. 

We now claim that $S'$ together with $F' := \inv_N(F(S'))$, $B' := \inv_N(B(S'))$, and $U' := \inv_N(U(S'))$ constitute a Morse decomposition for $S$. By definition, $S'$, $F'$, $B'$, and $U'$ are all invariant sets, which satisfies the first requirement of being a Morse decomposition. We will proceed by showing that $F'$, $B'$, and $U'$ are all isolated by $N$. But first, we will characterize the types of paths that can exist between simplices in $S'$, $F(S')$, $B(S')$, and $N(S')$. As $S$ is isolated by $N$, all paths between these sets must be contained in $N$. There are twelve possible types of paths in $S$ which originate at one of these sets and terminate at another. By definition, there cannot exist a path in $\rho \; : \; \mathbb{Z} \cap [0,n] \to S$ where $\rho( 0 ) \in S'$ and $\rho( n ) \in U(S')$ or vice versa. Similarly, there cannot exist a path from $S'$ to $B(S')$, or $S'$ is not isolated by $N$. By similar reasoning, there cannot exist a path from $F(S')$ to $B(S')$, or $S'$ is not isolated by $N$. Likewise, there can be no path from $F(S')$ to $S'$. Hence, there are seven remaining types of paths to consider. 

There cannot exist a path in $S$ from $\sigma \in U(S')$ to $\tau \in B(S')$, as if such a path existed, then there is necessarily a path in $S$ from $\sigma$ to some $\tau' \in S'$, which implies that $\sigma \in B(S')$. Similarly, there cannot exist paths from $\sigma \in F(S')$ to $\tau \in U(S')$, else there is necessarily a path from some $\tau' \in S'$ to $\tau$, which would imply $\tau \in F(S')$. We are left with five types of paths that are possible: paths from $B(S')$ to $S'$, $U(S')$, or $F(S')$, paths from $S'$ to $F(S')$, and paths from $U(S')$ to $F(S')$.  

Note that if $B'$ were not isolated, then there exists a path $\rho \; : \; \mathbb{Z} \cap [0,n] \to S$ such that $\rho( 0 ), \rho( n ) \in B'$, but there must exist some $i \in (0,n) \cap \mathbb{Z}$ such that $\rho( i ) \not\in B(S')$. But $S' \cup B(S') \cup F(S') \cup U(S') = S$, so it follows that $\rho(i)$ is in $F(S')$, $U(S')$, or $S'$. But there are no possible paths from one of these sets to $B$, so it follows that no such $\rho$ can exist, and it follows that $B'$ is isolated by $N$. Similar arguments imply that $F'$ and $U'$ are isolated by $N$. 

Hence, it remains to choose a partial order $\leq$ on $S'$, $B'$, $U'$, and $F'$. We choose the partial order given by the relations $S',U', F' \leq B'$, and $F' \leq U',S'$.  Because our choice of relations corresponds to possible connections, the third requirement for being a Morse decomposition follows immediately. Hence, $\md{} = \{ S', B', F', N' \}$ is a Morse decomposition for $S$, but some elements of $\md{}$ might be the emptyset. 

Now, consider $\sigma \in S \setminus S'$. Because $S'$ is isolated, it follows that $\alpha( \rho )$ or $\omega( \rho )$ is not contained in $S'$. If they both were, then $S'$ would not be isolated. Without loss of generality, assume that $\alpha( \rho )$ is not contained in $S'$. Then $\omega( \rho ) \subseteq B'$, so $B' \neq \emptyset$. Hence, $|\md{}| \geq 2$. 
\end{proof}

\begin{proposition}
Let $S$ denote an isolated invariant set in $N$ under $\mv{}$. If $S$ is minimal, then $S$ is strongly connected.
\label{prop:minimal-implies-strongly-connected}
\end{proposition}
\begin{proof}
Pick $\sigma \in S$. Then there exists an essential solution $\rho \; : \; \mathbb{Z} \to S$ where $\rho(0) = \sigma$. It follows by Proposition \ref{prop:alpha-omega-strongly-connected} that $\alpha( \rho )$ is a strongly connected invariant set. Hence, by Proposition \ref{prop:isolated-completion-strongly-connected}, $\iscomp_N( \alpha( \rho ) )$ is strongly connected. We claim that $\iscomp_N( \alpha( \rho )) = S$. By Proposition \ref{prop:is-comp-included}, $\iscomp_N( \alpha( \rho ) ) \subseteq S$. Hence, it remains to be shown that $S \subseteq \iscomp_N( \alpha( \rho ) )$. Aiming for a contradiction, assume that there exists a $\sigma \in S \setminus \iscomp_N( \alpha( \rho ) )$. Thus, by Proposition \ref{prop:morse-decomp-exists}, there exists a nontrivial Morse decomposition for $S$, and thus $S$ is not minimal. Hence, $S = \iscomp_N( \alpha( \rho ))$, so $S$ is strongly connected. 
\end{proof}

\begin{corollary}
An isolated invariant set is minimal if and only if it is strongly connected. 
\label{corollary:strongly-connected-minimal-equivalence}
\end{corollary}

Corollary \ref{corollary:strongly-connected-minimal-equivalence} immediately implies Proposition \ref{prop:min}. 

==> removed-changingn.tex <==
\section{Changing the Isolating Neighborhood}
\label{sec:chang}

In Section \ref{sec:persist} and Section \ref{sec:barcode}, we have always assumed that we are given a sequence of Conley-Morse graphs $G_1$, $G_2$, \ldots, $G_m$ which correspond to decompositions of isolated invariant sets $S_1$, $S_2$, \ldots, $S_n$ where each $S_i$ is isolated by some fixed $N$. With this assumption, we were able to develop a method to extract zigzag filtrations which capture the changing structure of a sequence of Conley-Morse graphs, and we developed a method that summarized how the Conley index changes across the vertices of the sequence of Conley-Morse graphs. In Section \ref{sec:barcode}, we used the barcodes from these zigzag filtrations to define a barcode for a sequence of Conley-Morse graphs, so long as they all correspond to decompositions of isolated invariant sets in a fixed $N$. In this section, we briefly generalize these results. In particular, we will instead assume that each $G_i$ corresponds to an isolated invariant set $S_i$ in an isolating neighborhood $N_i$. The primary task is to extract zigzag filtrations as we did in Section \ref{sec:persist}. Once we have the requisite filtrations, the techniques from Section \ref{sec:barcode} can be used as-is, giving us a barcode for a changing Conley-Morse graph. 

\subsection{Graph Structure Persistence}

First, we extend the results in Section \ref{sec:persist} to summarize the changing structure of the Conley-Morse graph. As in Section \ref{sec:persist}, we will focus our attention on two Conley-Morse graphs $G_1$ and $G_2$ with corresponding Morse decompositions $\md{1}$ and $\md{2}$ for isolated invariant sets $S_1$ and $S_2$. However, now we assume that $S_1$ and $S_2$ are isolated by isolating neighborhoods $N_1$ and $N_2$, respectively. 

\begin{proposition}
Let $M_1$ denote an isolated invariant set in $N_1$ under $\mv{1}$ and $M_2$ denote a minimal Morse set in $N_2$ under $\mv{2}$, where $N_2\subseteq N_1$ and $\mv{2} \sqsubseteq \mv{1}$. If $M_1 \cap M_2 \neq \emptyset$, then $M_2 \subseteq M_1$.
\label{prop:mdsubextended}
\end{proposition}
\begin{proof}
If $M_1 \cap M_2 \neq \emptyset$, then there exists $\sigma \in M_1 \cap M_2$. Pick some $\tau$ in $M_2$. Note that as $M_2$ is a minimal Morse set, then by Lemma \ref{lem:path} there must exist paths $\rho \; : \; [0,p] \to N_2$ and $\rho' \; : \; [p,q] \to N_2$ under $\mv{2}$ where $\rho(0) = \rho'(q) = \sigma$ and $\rho(p) = \rho'(p) = \tau$. We have that $N_2 \subseteq N_1$, so $\rho$ and $\rho'$ are also paths in $N_1$ under $\mv{2}$. Furthermore, by Lemma \ref{lem:min}, $\rho$ and $\rho'$ are paths in $N_1$ under $\mv{1}$. Hence, $\tau \in M_1$, as if $\tau \not\in M_1$, then $M_1$ is not isolated, a contradiction. This implies that $M_2 \subseteq M_1$.  
\end{proof}

Hence, given $G_1$ and $G_2$ which correspond to Morse decompositions of isolated invariant sets $S_1$ and $S_2$ in $N_1$ and $N_2$ under $\mv{1}$ and $\mv{2}$, one can construct a Conley-Morse graph $G_{1,2}$ for the minimal Morse decomposition of the maximal invariant set in $N_1 \cap N_2$ under $\mvint{1}{2}$. We again get partial functions $\iota_1 \; : \; V(G_{1,2}) \to V(G_1)$ and $\iota_2 \; : \; V(G_{1,2}) \to V(G_2)$. The notions of a relevant vertex, relevant connection, the relevant Conley-Morse graph generalize naturally to this setting, so we instead take $G_{1,2}$ to be the relevant Conley-Morse graph with respect to $G_1$ and $G_2$. A direct analog of Proposition \ref{prop:edgepreserving} holds, which implies that $\iota_1$ and $\iota_2$ are edge preserving. Hence, by using the Dowker sink complex, we get a zigzag filtration in Equation \ref{eqn:simple-graph-pers-changing-n}. 
\begin{equation}
    \ds(G_1) \leftarrow \ds(G_{1,2}) \rightarrow \ds(G_2)
    \label{eqn:simple-graph-pers-changing-n}
\end{equation}
This naturally extends to the more general zigzag filtration in Equation \ref{eqn:complex-graph-pers-changing-n}. 
\begin{equation}
    \ds(G_1) \leftarrow \ds(G_{1,2}) \rightarrow \ds(G_2) \leftarrow \ds(G_{2,3}) \rightarrow \cdots \leftarrow \ds(G_{n-1,n}) \rightarrow \ds(G_n)
    \label{eqn:complex-graph-pers-changing-n}
\end{equation}
Hence, we have a zigzag filtration which capture the changing Conley-Morse graph under variable $N$. 

\subsection{Conley Index Persistence}

We now move to computing the persistence of the Conley Index when $N$ is not fixed. Let $G_1$ and $G_2$ denote Conley-Morse graphs for isolated invariant sets $S_1$ and $S_2$ in isolating neighborhoods $N_1$ and $N_2$. In general, if $(P_1,E_1)$ and $(P_2,E_2)$ are index pairs in $N_1$ and $N_2$, it does not follows that $(P_1 \cap P_2, E_1 \cap E_2)$ is an index pair in $N_1 \cap N_2$. The authors in \cite{DMS2020} got around this problem by instead requiring that isolated invariant sets be isolated by $N_1 \cup N_2$. In this setting, we do not assume that we can choose our isolating neighborhood, which was done in \cite{DMS2020}. Hence, we need a different approach. 

We will consider the relevant Conley-Morse graph of the minimal Morse decomposition for the maximal invariant set in $N_1 \cap N_2$, which we denote $G_{1,2}'$. Note that if a Morse set $M \in G_{1,2}'$ is isolated by $N_1 \cap N_2$, it does not necessarily follow that $M$ is isolated by $N_1$ or $N_2$. However, if $M \in G_1$ satisfies $M \subseteq N_1 \cap N_2$, then $M$ must be isolated by $N_1 \cap N_2$. Hence, instead we focus on a different setting. Consider $M_1 \in V(G_1)$ and $M_2 \in V(G_2)$ where $M_1, M_2 \subseteq N_1 \cap N_2$. Methods in Section \ref{sec:chang} can be used to compute index pairs $(P_1,E_1)$ in $N_1$ and $(P_2,E_2)$ in $N_2$ for $M_1$ and $M_2$. We use the next proposition to find index pairs in $N_1 \cap N_2$. 
\begin{proposition}
Let $S$ denote an isolated invariant set in isolating neighborhoods $N$ under $\mv{}$. Furthermore, let $(P,E)$ denote an index pair for $S$ in $N$, and let $N' \subseteq N$ be a closed set. If $P \setminus E \subseteq N'$, then $(P \cap N', E \cap N')$ is an index pair for $S$ in $N'$ under $\mv{}$. 
\label{prop:subsetn}
\end{proposition}
\begin{proof}
Consider $\sigma \in P$. Because $(P,E)$ is an index pair in $N$, we have that $F_{\mv{}}(P) \cap N \subseteq P$. $P \cap N' \subseteq P$, so it follows that $F_{\mv{}}( P \cap N' ) \cap N \subseteq P$. If $A \subseteq B$, then $A \cap C \subseteq B \cap C$. Hence, it follows that $F_{\mv{}}( P \cap N' ) \cap N \cap N' \subseteq P \cap N'$. Equivalently, since $N' \subseteq N$, we get that $F_{\mv{}}( P \cap N' ) \cap N' \subseteq P \cap N'$. The same argument also implies that $F_{\mv{}}( E \cap N' ) \cap N' \subseteq E \cap N'$. 

Now, we aim to show that $F_{\mv{}}( (P \cap N') \setminus (E \cap N') ) \subseteq N'$. Recall that $P \setminus E \subseteq N'$ and $E \subseteq P$. Hence, if $\sigma \in P$ but $\sigma \not\in P\cap N'$, then $\sigma \not\in P \setminus E$, so it follows that $\sigma \in E$. Thus, it follows that $(P \setminus E) = (P \cap N') \setminus (E \cap N')$. Hence, it is sufficient to consider $F_{\mv{}}( P \setminus E)$. Fix $\sigma \in P \setminus E$, and fix $\tau \in F_{\mv{}}( \sigma )$. Either $\tau \in \cl( \sigma )$ or $\tau \in [ \sigma ]_{\mv{}}$. If $\tau \in \cl( \sigma )$, then $\tau \in N'$, as $\cl( \sigma )$ is the intersection of all closed sets which contain $\sigma$, and $N'$ is by assumption a closed set which contains $\sigma$. Hence, $\tau \in N'$. Thus, assume that $\tau \in [ \sigma ]_{\mv{}}$. Aiming for a contradiction, assume that $\tau \not\in N'$. But because $(P,E)$ is an index pair, and $(P \cap N') \setminus ( E \cap N' ) = P \setminus E$, it follows that $\tau \in N$. Similarly, $(P,E)$ is an index pair, and because $\sigma \in P$ and $\tau \in F_{\mv{}}( \sigma ) \cap N$, it follows that $\tau \in P$. But $(P \setminus E) \subseteq N'$, and $E \subseteq P$, so it follows that $\tau \in E$. By assumption, $[ \sigma ]_{\mathcal{V}} = [ \tau ]_{\mathcal{V}}$. Thus, $\sigma \in F_{\mathcal{V}}( \tau )$. The fact that $(P,E)$ is an index pair implies that $F_{\mv{}}( E ) \cap N \subseteq E$. However, $\tau \in E$, and $F_{\mv{}}( \tau ) \cap N \cap (P \setminus E) \neq \emptyset$. This is a contradiction, so $\tau$ must be an element of $N'$. 
\end{proof}
This proposition allows us to tweak the strategy in Section \ref{sec:persist} to find filtrations for the changing Conley index when the isolating neighborhood is not fixed. In Section \ref{sec:persist}, we considered all ``maximal'' sequences $\{ (P_i, E_i) \}_{i = a}^b$, where $(P_i, E_i)$ is an index pair for a Morse set represented as a vertex in the Graph $G_i$, and for all $i$ we have that $(P_i \setminus E_i ) \cap (P_{i+1} \setminus E_{i+1}) \neq \emptyset$. The maximality condition requires that there cannot exist index pairs $(P_{a-1}, E_{a-1})$ or $(P_{b+1},E_{b+1})$ such that $(P_{a-1} \setminus E_{a-1}) \cap (P_a \setminus E_a) \neq \emptyset$ or $(P_{b+1} \setminus E_{b+1}) \cap (P_b \setminus E_b) \neq \emptyset$.

It is instructive to consider two Conley-Morse graphs $G_1$, $G_2$, which correspond to Morse decompositions $\md{1}$, $\md{2}$ of isolated invariant sets $S_1$,$S_2$ in $N_1$, $N_2$ under $\mv{1}$, $\mv{2}$. Each $M_1 \in \md{1}$ and $M_2 \in \md{2}$ is associated with a single index pair in $N_1$ or $N_2$. We use $(P_1, E_1)$ and $(P_2, E_2)$ to denote index pairs for $M_1 \in \md{1}$ and $M_2 \in \md{2}$. In Section \ref{sec:persist}, we took all pairs of index pairs $(P_1,E_1)$ and $(P_2,E_2)$, and if $(P_1 \setminus E_1) \cap (P_2 \setminus E_2) \neq \emptyset$, we consider the filtration in Equation \ref{eqn:changing-n-wrong}.
\begin{equation}
    (P_1,E_1) \supseteq (P_1 \cap P_2, E_1 \cap E_2) \subseteq (P_2, E_2)
    \label{eqn:changing-n-wrong}
\end{equation}
However, if $(P_1, E_1)$ is an index pair in $N_1$ and $(P_2,E_2)$ is an index pair in $N_2$, then $(P_1 \cap P_2, E_1 \cap E_2)$ need not be an index pair in $N_1 \cap N_2$. Thus, by extracting the barcode, we are not actually computing a changing Conley index.

However, if $(P_1 \setminus E_1) \subseteq N_1 \cap N_2$ and $(P_2 \setminus E_2) \subseteq N_1 \cap N_2$, then by applying Proposition \ref{prop:subsetn}, we obtain the index pairs $(P_1 \cap N_1 \cap N_2, E_1 \cap N_1 \cap N_2)$ and $(P_2 \cap N_1 \cap N_2, E_2 \cap N_1 \cap N_2)$ in $N_1 \cap N_2$. Note that these are both index pairs in $N_1 \cap N_2$, so by Theorem \ref{thm:interindexpair}, the pair $(P_1 \cap P_2 \cap N_1 \cap N_2, E_1 \cap E_2 \cap N_1 \cap N_2)$ is also an index pair in $N$. We use this index pair to obtain the zigzag filtration in Equation \ref{eqn:changing-n-short}. 
\begin{equation}
    (P_1,E_1) \supseteq ( P_1 \cap P_2 \cap N_1 \cap N_2, E_1 \cap E_2 \cap N_1 \cap N_2 ) \subseteq (P_2, E_2)
    \label{eqn:changing-n-short}
\end{equation}
Note that all pairs in this zigzag filtration are index pairs, so by extracting the barcode, one is actually computing a changing Conley index. The approach naturally extends to the case when one has more than two Conley-Morse graphs. 

In Section \ref{sec:persist}, we found all possible sequences $\{(P_i,E_i)\}$ such that $(P_i,E_i)$ is the index pair for a Morse set $M \in \md{i}$ and $(P_i \setminus E_i ) \cap (P_{i+1} \setminus E_{i+1}) \neq \emptyset$. When $N$ is variable, we need a slightly different approach. Instead, we find all possible sequences $\{(P_i,E_i)\}$ such that $(P_i \setminus E_i) \subseteq N_{i} \cap N_{i+1}$, $(P_i \setminus E_i) \subseteq N_{i-1} \cap N_i$, and $(P_i \setminus E_i) \cap (P_{i+1} \setminus E_{i+1}) \neq \emptyset$. The former two equations guarantee that each extracted zigzag filtration represents a changing Conley index, while the third reduces the number of possible filtrations to those where classes can persist. We then get a set of filtrations of the type in Equation \ref{eqn:changing-n-long}. 
\begin{equation}
    (P_1,E_1) \supseteq ( P_1 \cap P_2 \cap N_1 \cap N_2, E_1 \cap E_2 \cap N_2 \cap N_3 ) \subseteq (P_2, E_2) \supseteq \ldots \subseteq (P_n,E_n)
    \label{eqn:changing-n-long}
\end{equation}
The techniques in Section \ref{sec:barcode} can then be used to eliminate redundancies and to extract a barcode which corresponds to a sequence of Conley-Morse graphs. 

==> removed-conleyindexinter.tex <==
\subsubsection{Intersecting Index Pairs}

Before we present our technique for extracting zigzag filtrations from Conley-Morse graphs, we briefly elaborate on Theorem \ref{thm:interindexpair}. For index pairs $(P_1,E_1)$ and $(P_2, E_2)$ in $N$ under $\mathcal{V}_1$ and $\mathcal{V}_2$, this allows us to link $\inv( P_1 \cap P_2 \setminus (E_1 \cap E_2))$ to the \sout{minimal} Conley-Morse graph for the maximal isolated invariant set under $\mvint{1}{2}$. We begin by establishing some terminology.

\begin{definition}
Let $S$ be an invariant set in a closed set $N$. The \emph{isolated completion} of $S$ in $N$ is the smallest isolated invariant set $S'$ in $N$ such that $S \subseteq S'$.
\end{definition}
\tamal{Isolated completion of $S$ in $N$ is denoted as $\iscomp_N(S)$ which is easy to compute.} 
\begin{proposition}
Let $S$ be an invariant set in $N$. Then $\iscomp_N(S) = S \cup R$, where $R$ is the is the image of the set of paths $\rho \; : \; \mathbb{Z}\cap[0,n] \to N$ such that $\rho(0), \rho(n) \in S$.
\label{prop:iscomp-paths}
\end{proposition}
\begin{proof}
Note that $\iscomp_N(S)$ necessarily contains $S$, and if there exists a $\rho \; : \; \mathbb{Z}\cap[0,n] \to N$ such that $\rho(0), \rho(n) \in S$ and $\im( \rho ) \not\subset \iscomp_N(S)$, then $\iscomp_N(S)$ is not isolated. Axiomatically, each $\sigma \in S$ is part of an essential solution that is contained in $S$. If $\sigma = \rho(i)$, then we construct an essential solution $\rho'$ such that $\rho'(i) = \sigma$. As $\rho( 0 ),\rho(n) \in S$, there must exist essential solutions $r_0, r_n \; : \; \mathbb{Z} \to S$ such that $r_0( 0 ) = \rho(0)$ and $r_n( n ) = \rho(n)$. Thus, we let $\rho'(j) := r_0(j)$ if $j \leq 0$, $\rho'(j) = \rho( j )$ if $0 \leq j \leq n$, and $\rho'(n) = r_n(j)$ if $j \geq n$. Thus, $\sigma = \rho'(i)$, so $S \cup R$ is an invariant set. Thus, we have shown that $S \cup R$ is the smallest isolated invariant set which contains $S$, so $\iscomp_N(S) = S \cup R$. 
\end{proof}

\tamal{We are in particular interested in the case of the minimal Morse decomposition.} 

\begin{proposition}
Let $S \subseteq N$ denote an invariant set, and let $S'$ denote an isolated invariant set in $N$. If $S \subseteq S'$, then $\iscomp_N(S) \subseteq S'$. 
\label{prop:is-comp-included}
\end{proposition}
\begin{proof}
By Proposition \ref{prop:iscomp-paths}, $\iscomp_N(S) = S \cup R$, where $R$ is the set of paths in $N$ which originate and terminate in $S$. Consider such a path $\rho \; : \; [0,n] \cap \mathbb{Z} \to N$, where $\rho(0) \in S \subseteq S'$ and $\rho( n ) \in S \subseteq S'$. By assumption, $S'$ is isolated, so it follows that for all $i \in [0,n] \cap \mathbb{Z}$, $\rho(i) \in S'$. Hence, $S \subseteq S'$ and $R \subseteq S'$, so it follows that $\iscomp_N( S ) \subseteq S'$. 
\end{proof}

\begin{proposition}
Let $S$ denote an isolated invariant set in $N$, and let $\mathcal{A}$ denote the set of Morse sets $M$ in the minimal Morse decomposition for $\inv(N)$ where $M \subseteq S$. Then, $S = \iscomp_N( \cup_{M \in \mathcal{A}} M )$. 
\label{prop:indexpairiscomp}
\end{proposition}
\begin{proof}
For notational ease, we let $S' = \cup_{M \in \mathcal{A}} M$. By Proposition \ref{prop:is-comp-included}, it follows immediately that $\iscomp_N( S' ) \subseteq S$. Hence, we aim to show that $S \subseteq \iscomp_n( S' )$. Aiming for a contradiction, let $\sigma \in S \setminus \iscomp_n( S' )$. Note that $\sigma \not\in \iscomp_N(S')$, and by Proposition \ref{prop:iscomp-paths}, $\iscomp_N(S') = S' \cup R$, where $R$ is the set of paths originating and terminating in $S'$. So, $\sigma \not\in R$. But, $S$ is an invariant set, so there must exist some essential solution $\rho \; : \; \mathbb{Z} \to S$ where $\rho( 0 ) = \sigma$. Note too that there cannot exist both an $i^- < 0$ and an $i^+ > 0$ where $\rho( i^{-} ) \in M \in \mathcal{A}$ and $\rho( i^+ ) \in M' \in \mathcal{A}$. If there existed such a pair, then $\sigma$ would be on a path between $M$ and $M'$, but $\sigma \not\in R$. 

Because $\rho( \sigma ) = 0$, $\sigma$ is part of the maximal invariant set in $N$. By the definition of the minimal Morse decomposition, it follows that $\sigma$ is either in a minimal Morse set $M$, or $\sigma$ is on a path between minimal Morse sets $M$ and $M'$. If $\sigma$ is in a minimal Morse set $M$, then $M \not\in A$, because $\sigma\not\in S'$. Hence, $M \cap S \neq \emptyset$, but $M \not\subseteq S$. This contradicts Proposition \ref{prop:mdsub}. Hence, $\rho$ restricts to a path such that $\sigma$ is on a path between two Morse sets, which we denote $M$ and $M'$, and at least one of $M$ and $M'$ is not in $\mathcal{A}$. In addition, at least one of $M$ and $M'$ is not in $S$ by definition of $A$. But, this implies that $\rho( \mathbb{Z} ) \not\in S$, a contradiction. 
\end{proof}

We strengthen the result in Theorem \ref{thm:interindexpair} with the following corollary. 

\begin{corollary}
Let $(P_1, E_1)$, $(P_2, E_2)$ denote index pairs in $N$ for isolated invariant sets under $\mv{1}$, $\mv{2}$, and let $S = \cup_i S_i$ denote the union of all \sout{minimal} \tamal{I dont think minimal is necessary here, no?} isolated invariant sets in $(P_1 \cap P_2) \setminus (E_1 \cap E_2)$ which are isolated by $N$. The pair $(P_1 \cap P_2, E_1 \cap E_2)$ is an index pair in $N$ for $\iscomp_N(S)$. 
\label{cor:morseset}
\end{corollary}
\begin{proof}
By Theorem \ref{thm:interindexpair}, $(P_1 \cap P_2, E_1 \cap E_2)$ is an index pair in $N$ for $S' := \inv( (P_1 \cap P_2 ) \setminus ( E_1 \cap E_2 ) )$. Theorem \ref{thm:interisolated} implies that $S$ is an isolated invariant set. Finally, Proposition \ref{prop:indexpairiscomp} implies that $S' = \iscomp_N( S )$. 
\end{proof}
This result provides a description of the invariant set for the index pair $(P_1 \cap P_2, E_1 \cap E_2)$. But in this paper, we are trying to compute the persistence of the Conley-Morse graph. Hence, we aim to relate the set $\iscomp_N(S)$ to the Conley-Morse graph. Given a Conley-Morse graph $G$, each vertex and edge is associated with a set of simplices. In the case of a vertex $v \in V(G)$, the vertex $v$ corresponds to a Morse set $M$. We denote this relationship by writing $\simps(u) = M$. Edges, in contrast, correspond to all simplices which lie on a direct connection between two Morse sets. Formally, we consider an edge $(u,v) \in E(G)$ where $u$ corresponds to the Morse set $M$ and $v$ corresponds to the Morse set $M'$. We define $\simps(u,v) = \{ \im( \rho ) \; | \; \rho \text{ a connection from } M \text{ to } M'\} \setminus (M \cup M')$. 
\begin{theorem}
Let $(P_1, E_1)$, $(P_2, E_2)$ denote index pairs in $N$ for isolated invariant sets under $\mv{1}$, $\mv{2}$, and let $G$ denote the Conley-Morse graph for the minimal Morse decomposition of the maximal invariant set in $N$ \tamal{under which vector field? I guess intersected field}. Furthermore, let $V$ denote the set of vertices $v$ in $V(G)$ for which $\simps(v) \subseteq (P_1 \cap P_2)\setminus(E_1 \cap E_2)$, and let $E$ denote the the set of edges $\{ (u,v) \in E(G) \; | \; u,v \in V \}$. 
The pair $(P_1 \cap P_2, E_1 \cap E_2)$ is an index pair in $N$ for \[\left(\bigcup\limits_{v \in V}{\simps( v )}\right) \bigcup \left(\bigcup\limits_{(u,v) \in E}{ \simps(u,v) }\right).\]
\label{thm:correspond}
\end{theorem}
\begin{proof}
By Corollary \ref{cor:morseset}, $(P_1 \cap P_2, E_1 \cap E_2)$ is an index pair for the isolated completion of $S = \cup_{v \in V} \simps(v)$. Let $\rho \; : \; [0,n] \cap \mathbb{Z} \to N$ denote a direct connection from $S$ to itself. In particular, assume that $\rho$ connects the Morse set corresponding to vertex $u$ to that Morse set corresponding to vertex $v$. Hence, there must be an edge $(u,v) \in E$ which contains exactly those simplices on direct path from the Morse set corresponding to $u$ to the Morse set corresponding to $v$. Thus, $E$ contains exactly those simplices on connections from $S$ to itself, which by Proposition \ref{prop:iscomp-paths} is the same as the isolated completion.  
\end{proof}
